Exploring The Role of Mean Teachers in Self-supervised Masked Auto-Encoders

Masked image modeling (MIM) has become a popular strategy for self-supervised learning~(SSL) of visual representations with Vision Transformers. A representative MIM model, the masked auto-encoder (MAE), randomly masks a subset of image patches and reconstructs the masked patches given the unmasked patches. Concurrently, many recent works in self-supervised learning utilize the student/teacher paradigm which provides the student with an additional target based on the output of a teacher composed of an exponential moving average (EMA) of previous students. Although common, relatively little is known about the dynamics of the interaction between the student and teacher. Through analysis on a simple linear model, we find that the teacher conditionally removes previous gradient directions based on feature similarities which effectively acts as a conditional momentum regularizer. From this analysis, we present a simple SSL method, the Reconstruction-Consistent Masked Auto-Encoder (RC-MAE) by adding an EMA teacher to MAE. We find that RC-MAE converges faster and requires less memory usage than state-of-the-art self-distillation methods during pre-training, which may provide a way to enhance the practicality of prohibitively expensive self-supervised learning of Vision Transformer models. Additionally, we show that RC-MAE achieves more robustness and better performance compared to MAE on downstream tasks such as ImageNet-1K classification, object detection, and instance segmentation.

==> 5_discussion.tex <==
\section{Discussion and Limitations}
As shown in \cref{tab:rc}, the iteration time of RC-MAE is slower than MAE. 
It is due to the fact that the self-distillation architecture needs an extra teacher network to MAE and thus it requires more computation cost.
Therefore, there is a tradeoff between accuracy and speed.
We leave the future works to accelerate the training time of the RC-MAE.

==> fig/cosine.tex <==
\begin{figure}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\linewidth]{fig/cos_dist.pdf}
\end{center}
% \vspace{-0.05in}
\caption{\textbf{Cosine distribution between reconstruction and consistency gradients.}}
\label{fig:cos}
% \vspace{-0.3in}
\end{figure}

==> fig/epoch.tex <==
% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=0.7\linewidth]{fig/comparison_epoch.pdf}
% \end{center}
% \caption{\textbf{Fine-tuning top-1 accuracy curve: RC-MAE~(800epch) vs. MAE~(1600ep).}}
% \label{fig:epoch}
% \end{figure}


\begin{wrapfigure}{r}{7.1cm}
\vspace{-5mm}
\includegraphics[width=1.0\linewidth]{fig/comparison_epoch.pdf}
\vspace{-0.75cm}
\caption{\textbf{Fine-tuning top-1 accuracy curve: RC-MAE~(800epoch) vs. MAE~(1600epoh).}
RC-MAE achieves comparable accuracy~(83.4\%) compared to MAE trained for longer 1600 epoch.
}
\vspace{-0.3cm}
\label{fig:epoch}
\end{wrapfigure} 

==> fig/loss.tex <==
\begin{figure}[t]
\begin{center}
% \scalebox{0.68}{
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=1.0\linewidth]{fig/loss_comp.pdf}
% }
\end{center}
% \vspace{-0.05in}
\caption{\textbf{Reconstruction loss comparison.} 
RC-MAE-S uses the \textbf{S}ame mask patches for both student and teacher networks, while RC-MAE-D uses the \textbf{D}ifferent mask patches. 
The reconstruction loss of RC-MAE-D is higher than that of MAE, but RC-MAD-D outperforms MAE in downstream tasks \eg, ImageNet fine-tuning. 
This suggests that RC-MAE-D yields a regularization effect, preventing overfitting.
If unspecified, RC-MAE means RC-MAE-S in the rest of this paper.}
\label{fig:loss}
% \vspace{-0.3in}
\end{figure}

==> tab/ab.tex <==
\begin{table}
  \begin{minipage}{.47\textwidth}
    \centering
    \caption{\textbf{Comparison between Student vs. Teacher networks} on ImageNet-1K evaluation. FT and LN denote fine-tuning and linear probing top-1 accuracies, respectively.}
    \begin{tabular}{lcc}
    \toprule
    Checkpoint & FT & LN \\
%     \multicolumn{1}{c}{\multirow{2}[4]{*}{Checkpoint}} & \multicolumn{2}{c}{FT} & \multicolumn{2}{c}{LN} \\
% \cmidrule{2-5}          & top-1 & top-5 & top-1 & top-5 \\
    \midrule
    Student & 83.48  & 68.38  \\
    Teacher & \textbf{83.58}   & \textbf{68.41}   \\
    \bottomrule
    \end{tabular}%
    % \vspace{+0.25cm}
  \label{tab:teacher}%
  \end{minipage}%
  \hfill%
  \begin{minipage}{.47\textwidth}
    \centering
    \caption{\textbf{Training epoch comparison} using ViT-B.}
    \begin{tabular}{lccc}
    \toprule
    Method & Epoch & FT & LN \\
    \midrule
    MAE   & \multirow{2}[2]{*}{800} & 83.2   & 65.4  \\
    \textbf{RC-MAE} &       & \textbf{83.4}  & \textbf{66.3}  \\
    \midrule
    MAE   & \multirow{2}[2]{*}{1600} & 83.4  & 67.3 \\
    \textbf{RC-MAE} &       & \textbf{83.6}  & \textbf{68.4}  \\
    \bottomrule
    \end{tabular}%
    \label{tab:epoch}%
  \end{minipage}
\end{table}


==> tab/det.tex <==
\begin{table}[t]
\caption{\textbf{COCO object detection and segmentation} using Mask R-CNN with ViT-Base backbone. 
  For fair comparison, we follow the benchmarking transfer learning protocol~\citep{li2021benchmarking}.
}
  \centering
    % \begin{adjustbox}{width=\columnwidth, center}
    \scalebox{0.9}{
    \begin{tabular}{llcc}
    \toprule
    Method & Pre-Train Data & AP\textsuperscript{box} & AP\textsuperscript{mask} \\
    \midrule
    Superivsed~\citep{he2022mae} & IN1K w/ labels & 47.9  & 42.9 \\
    MoCo v3~\citep{chen2021mocov3} & IN1K  & 47.9  & 42.7 \\
    BEiT~\citep{bao2021beit}  & IN1K+DALLE & 49.8  & 44.4 \\
    MSN~\citep{assran2022msn} & IN1K & 46.6 & 41.5 \\
    iBOT~\citep{zhou2021ibot} & IN1K & 47.3 & 42.2 \\
    MAE~\citep{he2022mae}   & IN1K  & 50.3  & 44.9 \\
    \midrule
    % MAE~(our impl.) & IN1K  & 50.3  & 53.3 \\
    \rowcolor{teagreen}\textbf{RC-MAE~(ours)} & IN1K  & \textbf{51.0}  & \textbf{45.4} \\
    \bottomrule
    \end{tabular}%
    }
    \vspace{-0.5cm}
    % \end{adjustbox}
  \label{tab:det}%
\end{table}%


==> tab/epoch.tex <==
\begin{table}[t]
  \caption{\textbf{Training epoch comparison using ViT-B.}}
    \centering
    \begin{tabular}{lcccc}
    \toprule
    Method & Epoch & FT & LN & GPU Time~(h) \\
    \midrule
    MAE   & \multirow{2}[2]{*}{800} & 83.2   & 65.4 &125.5  \\
    \textbf{RC-MAE} &       & \textbf{83.4}  & \textbf{66.3} & 166.6  \\
    \midrule
    MAE   & \multirow{2}[2]{*}{1600} & 83.4  & 67.3 &256.5 \\
    \textbf{RC-MAE} &       & \textbf{83.6}  & \textbf{68.4} &331.1  \\
    \bottomrule
    \end{tabular}%
  \label{tab:epoch}%
\end{table}%


% \begin{table}[t]
%   \caption{\textbf{Training epoch comparison using ViT-B.}}
%     \centering
%     \begin{tabular}{lccc}
%     \toprule
%     Method & Epoch & FT & LN \\
%     \midrule
%     MAE   & \multirow{2}[2]{*}{800} & 83.2   & 65.4  \\
%     \textbf{RC-MAE} &       & \textbf{83.4}  & \textbf{66.3}  \\
%     \midrule
%     MAE   & \multirow{2}[2]{*}{1600} & 83.4  & 67.3 \\
%     \textbf{RC-MAE} &       & \textbf{83.6}  & \textbf{68.4}  \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:epoch}%
% \end{table}%


% \begin{table}[t]
%   \caption{\textbf{Training epoch comparison using ViT-B.}}
%   \centering
%     \begin{tabular}{lccccc}
%     \toprule
%     \multicolumn{1}{c}{\multirow{2}[4]{*}{Checkpoint}} & \multirow{2}[4]{*}{Epoch} & \multicolumn{2}{c}{FT} & \multicolumn{2}{c}{LN} \\
% \cmidrule{3-6}          &       & top-1 & top-5 & top-1 & top5 \\
%     \midrule
%     MAE   & \multirow{2}[2]{*}{800} & 83.2  & 96.4  & 65.4  & 86.0 \\
%     \textbf{RC-MAE} &       & \textbf{83.4}  & \textbf{96.6}  & \textbf{66.3}  & \textbf{86.6} \\
%     \midrule
%     MAE   & \multirow{2}[2]{*}{1600} & 83.4  & 96.5  & 67.3  & 87.3 \\
%     \textbf{RC-MAE} &       & \textbf{83.6}  & \textbf{96.6}  & \textbf{68.4}  & \textbf{87.9} \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:epoch}%
% \end{table}%


==> tab/finetune.tex <==
\begin{table}[t]
    \caption{\textbf{End-to-end fine-tuning setting.}
    }
  \centering
  % \begin{adjustbox}{width=\columnwidth, center}
    \begin{tabular}{ll}
    \toprule
    Config & Value \\
    \midrule
    optimizer                               & AdamW \\
    optimizer momentum                      & $\beta_1, \beta_2=0.9, 0.999$ \\
    weight decay                            & 0.05 \\
    layer-wise lr decay~\citep{bao2021beit} & 0.65 \\    
    base learning rate                      & 5e-4 \\
    drop path~\citep{huang2016dpr}          & 0.1~(S,B), 0.2~(L) \\
    batch size                              & 1024 \\
    learning rate schedule                  & cosine decay \\
    warmup epochs                           & 5 \\
    % training epochs                         & 300~(S), 100~(B,L) \\
    training epochs                         & 100 \\
    % augmentation                            & RandAug(9, 0.5)~\citep{cubuk2020randaugment} \\
    augmentation                            & RandAug(9, 0.5) \\
    label smoothing                         & 0.1 \\
    mixup~\citep{zhang2018mixup}            & 0.8 \\
    cutmix~\citep{yun2019cutmix}            & 1.0 \\
    \bottomrule
    \end{tabular}%
  \label{tab:finetune}%
\end{table}%

==> tab/linear.tex <==
\begin{table}[t]
    \caption{\textbf{Linear probing setting.}
    }
  \centering
  % \begin{adjustbox}{width=\columnwidth, center}
    \begin{tabular}{ll}
    \toprule
    Config & Value \\
    \midrule
    optimizer                               & LARS~\citep{you2017large} \\
    base learning rate                      & 0.1 \\
    weight decay                            & 0 \\
    batch size                              & 16,384 \\
    learning rate schedule                  & cosine decay \\
    warmup epochs                           & 10 \\
    training epochs                         & 90 \\
    augmentation                            & RandomResizedCrop \\
    \bottomrule
    \end{tabular}%
  \label{tab:linear}%
\end{table}%

==> tab/mask.tex <==
\begin{table}[h]
  \centering
  \caption{\textbf{Different mask ratio.} GPU time means pre-training time.}
    \begin{tabular}{lcccc}
    \toprule
    Method & Epoch & mask ratio & FN & GPU time (hours) \\
    \midrule
    MAE   & 800   & 75\%  & 83.2  & 125.5 \\
    RC-MAE & 800   & 75\%  & 83.4  & 166.6 \\
    RC-MAE & 800   & 80\%  & 83.4  & 142.6 \\
    RC-MAE & 800   & 85\%  & 83.2  & 136.4 \\ \hline
    MAE   & 1600  & 75\%  & 83.4  & 256.5 \\
    RC-MAE & 1600  & 75\%  & 83.6  & 331.1 \\
    RC-MAE & 1600  & 80\%  & 83.5  & 283.3 \\
    \bottomrule
    \end{tabular}%
  \label{tab:mask}%
\end{table}%



==> tab/mem.tex <==
\begin{wraptable}{r}{45mm}
\vspace{-0.7cm}
\caption{GPU Memory and training iter time for ViT-L.}
\label{tab:memory}%
\resizebox{0.32\textwidth}{!}{
    \begin{tabular}{lrc}
    \toprule
    Method & Memory & Iter. time \\
    \midrule
    MAE   & 84G   & 0.24s \\
    MSN   & 183G  & 1.56s \\
    iBOT  & 227G  & 1.04s \\
    BootMAE & 92G   & 0.45s \\
    \textbf{RC-MAE} & 90G   & 0.31s \\
    \bottomrule
    \end{tabular}%
}
\vspace{-1.5cm}
\end{wraptable}

==> tab/rc.tex <==
\begin{table}[t]
    \caption{\textbf{Different mask types for the teacher network in RC-MAE.}
      The `\textbf{S}ame' means that the teacher network uses the same mask tokens as the student and `\textbf{D}iff.' is the opposite.
      FT and LN denote end-to-end fine-tuning and linear probing on ImageNet-1K, respectively.
      % We use Mask R-CNN for object detection.
      }
  \centering
  % \begin{adjustbox}{width=\columnwidth, center}
    \begin{tabular}{llcccc}
    \toprule
    Method & Mask & FT & LN & AP\textsuperscript{box} & AP\textsuperscript{mask} \\
    \midrule
    MAE    & -     & 83.4   &67.3 & 50.3  & 44.9 \\
    RC-MAE-\textbf{D} & \textbf{D}iff.  & 83.6  & \textbf{68.7}    & 50.7  & 45.2 \\
    RC-MAE-\textbf{S} & \textbf{S}ame   & \textbf{83.6}  &68.4  & \textbf{51.0}  & \textbf{45.4} \\
    \bottomrule
    \end{tabular}%
    % \end{adjustbox}
    % \vspace{+0.3cm}
  \label{tab:rc}%
\end{table}%


% \begin{table}[t]
%     \caption{\textbf{Different mask types for the teacher network in RC-MAE.}
%       The `\textbf{S}ame' means that the teacher network uses the same mask tokens as the student and `\textbf{D}iff.' is the opposite.
%       FT denotes end-to-end fine-tuning on ImageNet-1K, respectively.
%       We use Mask R-CNN for object detection.
%       }
%   \centering
%   % \begin{adjustbox}{width=\columnwidth, center}
%     \begin{tabular}{llccc}
%     \toprule
%     Method & Mask & FT & AP\textsuperscript{box} & AP\textsuperscript{mask} \\
%     \midrule
%     MAE    & -     & 83.4    & 50.3  & 44.9 \\
%     RC-MAE-\textbf{D} & \textbf{D}iff.  & 83.6     & 50.7  & 45.2 \\
%     RC-MAE-\textbf{S} & \textbf{S}ame & \textbf{83.6}   & \textbf{51.0}  & \textbf{45.4} \\
%     \bottomrule
%     \end{tabular}%
%     % \end{adjustbox}
%     % \vspace{+0.3cm}
%   \label{tab:rc}%
% \end{table}%


% \begin{table}[t]
%     \caption{\textbf{Different mask types for the teacher network in RC-MAE.}
%       The `\textbf{S}ame' means that the teacher network uses the same mask tokens as the student and `\textbf{D}ifferent' is the opposite.
%       FT denotes end-to-end fine-tuning on ImageNet-1K, respectively.
%       We use Mask R-CNN for object detection.
%       }
%   \centering
%   % \begin{adjustbox}{width=\columnwidth, center}
%     \begin{tabular}{llcccc}
%     \toprule
%     Method & Mask type & Time~(s/iter) & FT & AP\textsuperscript{box} & AP\textsuperscript{mask} \\
%     \midrule
%     MAE    & -     & 0.91 & 83.4    & 50.3  & 44.9 \\
%     RC-MAE-D & \textbf{D}ifferent  & 1.18 & 83.6     & 50.7  & 45.2 \\
%     RC-MAE-S & \textbf{S}ame & 1.18 & \textbf{83.6}   & \textbf{51.0}  & \textbf{45.4} \\
%     \bottomrule
%     \end{tabular}%
%     % \end{adjustbox}
%     % \vspace{+0.3cm}
%   \label{tab:rc}%
% \end{table}%

